A Review of the In-Network Computing and Its Role in the Edge-Cloud Continuum

Future networks are anticipated to enable exciting applications and industrial services ranging from Multisensory Extended Reality to Holographic and Haptic communication. These services are accompanied by high bandwidth requirements and/or require low latency and low reliability, which leads to the need for scarce and expensive resources. Cloud and edge computing offer different functionalities to these applications that require communication, computing, and caching (3C) resources working collectively. Hence, a paradigm shift is necessary to enable the joint management of the 3Cs in the edge-cloud continuum. We argue that In-Network Computing (INC) is the missing element that completes the edge-cloud continuum. This paper provides a detailed analysis of the driving use-cases, explores the synergy between INC and 3C, and emphasizes the crucial role of INC. A discussion on the opportunities and challenges posed by INC is held from various perspectives, including hardware implementation, architectural design, and regulatory and commercial aspects.

==> Content/challenges_opportunities_C4_backup.tex <==
\section{Challenges, Opportunities, and Future Research Directions}\label{Challenges}
\noindent The in-network computing concept is changing the way we perceive the next-generation networking infrastructure. We can now reevaluate where and when data is processed and cached, and how and what is communicated. This paradigm shift has its own challenges, from hardware implementation and architectural design to regulatory and commercial aspects; and its opportunities from autonomy to scalability and to applying AI within the network. In the following, we will review each challenge as well as the opportunities for future research. 

\subsection{Technical Challenges for INC}
\vspace{-3pt}
\subsubsection{Memory} \noindent Recently, the advances in programmable data plane devices open up many opportunities to offload operations or functionalities to the switches. However, the limited memory constraint of the switches remains a major challenge that many applications make struggles to deal with it. Besides, the applications mentioned in Section~\ref{sec:Usecases} face a clear trade-off between performance and memory usage. For instance, in the in-network cache scenario, the cache hit rate and the accuracy of sketches are directly determined by the memory size of the networking equipment~\cite{jin2017netcache, liu2016one}. Similarly, the memory exhaustion of the device directly leads to a slow down of the performance of applications such as load balancing~\cite{miao2017silkroad} and monitoring~\cite{narayana2017language}. Even the most basic function of switches, such as packet forwarding, can suffer from limited memory space. To tackle the memory constraint, one solution is the design of a switching ASIC with internal custom logic and wires for the external Dynamic Random Access Memory (DRAM) access. However, this proves to be costly due to the design of numerous parallel DRAM modules combined with a DRAM controller. Therefore, the on-switch external DRAM is not widely used by vendors in today’s single-chip switches. Another possible solution is to utilize the unused resources and DRAM of the data center networks. However, there are some technical challenges in terms of performance, fault tolerance, and load balancing, though the programmable switch memory can be extended in a cost-effective manner. For example, the work in \cite{kim2020unleashing} particularly explores the possibility of re-purposing the affordable DRAM installed on data center servers to expand the memory available on a switch’s data plane. Instead of building another switching ASIC with a custom external-DRAM-access capability, they simply reuse an existing programmable switching ASIC built only with on-chip memory. The proposed approach designs three remote memory primitives: remote packet buffer, remote lookup table, and remote state store, leveraging Remote Direct Memory Access (RDMA) operations. The experimental result shows that the proposed system achieves high performance in terms of bandwidth, causing a little latency cost and absolutely 0\%  CPU overhead.

\subsubsection{Power consumption} Power consumption of programmable devices is one of the key performance indicators that directly reflect the packet processing efficiency of the chip,  measured in million packets per second per Watt (Mpps/Watt)~\cite{pongracz2013cheap}.
%Therefore, it concerns the researchers in the field of INC. %
Unlike the traditional chips with a lower number of transistors and switching frequency, today’s chips are of smaller volume and embed a large number of transistors that allow them to leave a higher processing capacity. Hence, it leads to more power dissipation which directly reflects the computing time and generates additional cooling costs. To overcome this power dissipation, the work in \cite{yang2019switchagg} redesigned the routing switches. These switches operate in two modes: (i) sleep mode that reduces the leakage power, and (ii) low-power mode that reduces the dynamic power.


\subsection{Adding the control dimension to INC}
\noindent Even though a general theory of goal-oriented communication was put forward a decade ago~\cite{10.1145/2160158.2160161}, this has not been fully achieved yet. However, transitioning to goal-oriented communication is becoming more urgent since end-users have become \textbf{producers} and \textbf{consumers} of contents as their devices are now embedded with various sensors, which help in creating and collecting various types of data from different domains such as energy, agriculture, healthcare, transport, security, and smart homes, among others.  With the exponential growth of diverse IoT devices, as well as various applications (e.g., intelligent manufacturing, smart agriculture), the expectations for the performance, reliability, and security of networks are greater than ever. For example, an industrial control system requires a strict target of a 2 ms network delay and 1 ms jitter. While achieving a controllable and observable system with such target performance metrics has been studied over more than half a century, and various criteria have been developed, difficulties arise when they are straightforwardly applied to a networked system consisting of a large number of subsystems. To be more specific, it has been recognized that for large-scale networked systems, these criteria are usually computationally prohibitive.

To this end, INC has the potential to alleviate the complexities of networked control systems by recognizing that communication is not an end in itself but rather a means to achieve some goals of the communicating parties. 
%Focusing on goals provides a framework for addressing the problem of potential ``misunderstanding” during communication, where ``reliable communication” means overcoming any initial misunderstanding between parties towards achieving a given goal. Redefining the communication reliability also provides a new selection of data to be transported over the network.
%
% \begin{figure}
%     \centering
%     \includegraphics{}
%     \caption{A figure showing IoT network control together with goal-oriented networking.  Similar to Fig 1 of https://arxiv.org/abs/2103.05391}
%     \label{fig:my_label}
% \end{figure}
%

In this aspect, INC can enable 4C, which is the extension of 3C with the addition of physical controllers. The act of control, is the end result of a collection of functions that operate at the management plane, and includes the computing, caching, and communication (3C) functions and their coordination to ensure an efficient operation.  These controllers could be deployed as microservices and placed optimally within the infrastructure alongside the 3C functions. That's where INC can come into play. For instance, a lifecycle management function can be deployed close to a compute function to optimize the control and management of that function on the run, without the delay induced when having a remote management entity. 



%\subsection{Economic Aspects of INC in the NGNI}
\label{INC_business}
 \noindent 
 %Many promising and novel networking and communications technologies are not picked up by the industry due to the promised benefits not meeting the CAPEX and OPEX in the network.  The studies related to network expenditure can be mainly classified into two general categories: (1) identification of CAPEX and OPEX for a network in general, and (2) economic analysis of networks.
 
%First, INC will enable an enhanced distributed collaborative computing paradigm throughout the Cloud-Edge-Mist Continuum in the NGNI. Hence, in addition to supporting low latency applications, INC also has the potential to increase the network utilization. Network traffic often follows daily, hourly, weekly, and seasonal patterns. These patterns may require rapidly not only moving to but also the processing of traffic in less utilized links and INC-enabled routers. Since this rapid modification to the network is not trivial in traditional architectures, network administrators often overprovision their network resources, which increases the CAPEX in the network. For example, the bandwidth is selected to support the highest traffic across a single link. During nonpeak times, this bandwidth is not used and is, therefore, a cost that has no return on investment is incurred. Similarly, the main benefit of cloud computing has been the ability to access computing resources only when it is needed. In the NGNI, traffic can be engineered in near real-time to adjust the needs of the network traffic. This dynamic nature prevents network operators from unnecessary network capacity increases and, thus, produces CAPEX savings. Further studies are needed to quantify CAPEX/OPEX savings of INC in the NGNI. A study of this nature was performed for SDN in \cite{KARAKUS201881} and can be taken as a starting point.
 
 
%Second, as the owner of an INC device may be a single person, an institution, or a company providing other network services, the task of including them in a conventional centralized pricing system is not trivial. Considering the geographical dispersion of the nodes, their mobility, and potential flexibility in the QoS demands, a {\em dynamic} financial model is more suitable for the INC computing architecture. Note that in a simple dynamic pricing model, a computational node, which has processed an offloaded task, bills the edge device usually based on the processing time duration multiplied by a fixed cost per time processing unit. Depending on how far from the edge device the INC node is positioned, it may request an additional incentive that is proportionate to the reduction in latency provided by the shorter network propagation times.  
 

%An SDN with NFN can be considered in action in the pricing of INC with 3C/4C integration. 
%An interest request comprising of content and functions arrives at the first node in the data plane. Suppose both content and function exist at that node and there is enough available capacity. In that case, the task will be executed at that node if the node satisfies the controller’s incentive condition. A request message consisting of the bid for executing the task and obtaining 3C/4C resource status from the execution information base is sent from the node to the controller. Then, the controller computes the cost for the received task and compares it with the bid requested by the node. If the difference is not larger than a specific threshold, the controller sends a verifying message to the node to execute the task. Otherwise, the controller checks another node that satisfies the threshold value and computing capability and will rout the task to that node. Besides, the controller should assign tasks optimally to be executed at the nodes to minimize the overall network cost. 
 

%Additionally, nonmonetary incentives should also be considered for INC in the NGNI. Note that NGNI is expected to support AI applications by supporting their distributed computations. Consequently, INC devices can store these learned models for their future use. This is similar to the financial model used by mobile applications. Additionally, employing INC in the NGNI has indirect incentives to cloud providers and ISPs. Note that by offloading delay-sensitive control tasks from the cloud to local network elements that can perform the latency bounded processing in NGNI, the traffic will be reduced significantly in the cloud. As in-network processing is done within the network, it means that transactions are terminated within their path rather than reach an end-host, saving the latency introduced by the end-host. Throughput is another performance advantage of using INC, which is improved by increasing the packet processing rate using a class of switches, designed as pipelines, continuously moving data without stalls. Lower power consumption is another advantage of INC. Since the overhead of in-network computing is small, and network switches are part of a user’s network, knowing that most of the power consumption is already paid by packet forwarding causes INC to be power efficient. 


%Different dynamic incentive mechanisms, such as those based on deep learning and game theory, can be formulated and applied to incentivize computing nodes to collaborate on the computation of tasks. Tables~\ref{table:Challenges_Economics} presents a classification of some papers on the economics of INC in the Cloud-Edge-Mist Continuum according to regulatory, safety, and incentive mechanism aspects. Using Stackelberg game theory, the incentive mechanism for mobile crowdsensing is proposed in \cite{zhan2020incentive} by taking the mobile users’ own resource demand into the economic model. As different users will have different behavior, they will participate in the mobile crowdsensing on different levels. Moreover, a dynamic incentive mechanism based on a deep reinforcement learning approach is proposed without knowing the private information of the users. Thus, service providers can learn the optimal pricing strategy from game experience. In the NGNI, the controller, as the leader of a Stackelberg game, can split the caching and computational capacity for offloading data and content caching, as well as decide the price dynamically for these services.

  
%Based on Nash bargaining, \cite{tang2020communication} proposes an incentive mechanism for device-to-device communication with 3C resource sharing. In the incentive mechanism, users can reach an agreement that specifies how their devices perform the resource allocation and share the benefits. This mechanism always ensures fair payment by collecting the system information and solving a Nash bargaining problem in a centralized fashion. Such a mechanism may also be useful for INC in the NGNI where the controller can collect the information of the nodes to solve a Nash bargaining problem in a centralized way to assign fairness bids to computing nodes. 


%Finally, the incentives gained by INC should also be distributed in a trusted way throughout the Cloud-Edge-Mist Continuum. In this aspect, distributed ledger methods provide a trustworthy solution. Blockchains and distributed ledgers allow, in general, entities to issue payments directly to each other without requiring either party to be trustworthy. Blockchains have found applications in many domains, including networking. In \cite{9232928}, the authors proposed a blockchain radio access network (B-RAN) that aggregates wireless resources across different service providers and establishes a large network of subnetworks. Furthermore, B-RAN avoids the additional overhead of centralized resource allocation schemes, endorses economic incentives, and builds strong trust between service providers and clients.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[ht]
\centering
\captionsetup{format=hang}
\caption{Regulatory, Privacy, Safety, Commercial, Legal and Ethical Issues Classification}
\label{table:Challenges_RSE}
\begin{adjustbox}{width=\textwidth,center=\textwidth}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{\textbf{Papers}} & \multicolumn{2}{c|}{\textbf{Regulatory }}             & 
\multicolumn{2}{c|}{\textbf{Privacy }}             &
\multicolumn{1}{c|}{\textbf{Safety }}                                             & \multicolumn{3}{c|}{\textbf{Legal} \And \textbf{Ethical Issues} }  &  \multicolumn{1}{c|}  {\textbf{Commercial} }   \\ 
\cline{2-9}
                                   & \textbf{Distributed Learning}      & \textbf{Knowledge Transfer}        & \textbf{Privacy Protection}        & \textbf{Differential Privacy}        & \textbf{Secure Computation}      & \textbf{Data Ethics}               & \textbf{Applied Ethics}            & \textbf{Business Ethics}      &    \\ 
\hline
\cite{gao2021sedml}                                 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &                           &                           &                           & \\ 
\hline
\cite{9629226}                                  &                           & \checkmark &                           &                           & \checkmark &                           &                           &                          &  \\ 
\hline
\cite{anahideh2021choice}                                  &                           & \checkmark &                           &           \checkmark                &  &                           &                           &                           & \\ 
\hline
\cite{8662743}                                &                           &                           &                           &                           &                           & \checkmark & \checkmark &       &                     \\ 
\hline
\cite{9293092}                                &  \checkmark                 &                           &                           &                           &     \checkmark                      &  &     &  &                          \\ 
\hline
\cite{8768490}                                 &                           &                           & \checkmark & \checkmark & \checkmark &                           &                           &            &                \\ 
\hline
\cite{8789542}                                &                           & \checkmark & \checkmark &                       \checkmark    &  &                           &                           &                      &      \\
\hline
\cite{zhan2020incentive}&                           &  &   &                          &  &                           &                           &                      &     \checkmark  \\
\hline
\cite{tang2020communication}                                &                           &   &   &                          &  &                           &                           &                      & \checkmark  \\
\hline
\end{tabular}
} 
 \end{adjustbox}
\end{table*}



\begin{table*}
    \centering
    \caption{Regulatory, Privacy, Safety,Legal and Ethical Issues Table of Acronyms}
    \begin{tabular}{|c|c|}
    \hline
    \textbf{Acronym} & \textbf{Term} \\
    \hline
        ISP & Internet Service Provider \\
        \hline
        INC & In-Network Computing \\
        \hline
        NGNI & Next Generation Network Initiative \\
        \hline
        CEP & Complex Event Processing \\
        \hline
        AI & Artificial Intelligence \\
        \hline
        DL & Deep Learning \\
        \hline
        SEDML & Securely and Efficiently Harnessing Distributed Knowledge in Machine Learning \\
        \hline
        SLA & Service-Level Agreement \\
        \hline
    \end{tabular}
    \label{tab:Acronyms_RSE}
\end{table*}
 \subsection{Regulatory, Privacy, Safety, Legal and Ethical Issues}
 
 \subsubsection{Regulatory}
%No one person, company, organization, or government runs the Internet. It is a globally distributed network comprising many voluntarily interconnected autonomous networks. It operates without a central governing body with each constituent network setting and enforcing its own policies. The central pillar in distributed governance of the Internet is net neutrality. Net neutrality is the concept that all data traffic on a network should be treated indiscriminately, and internet service providers would be restricted from blocking, slowing down, or speeding up the delivery of online content at their discretion. The current debate surrounding net neutrality is principally about how ISPs should be regulated and what role the government should play in overseeing their network management practices. Today, some countries have regulations about ``net neutrality” for networking, but not about cloud computing, which has (probably) been the key to enable the development of a plethora of cloud applications, but has disintermediated the telecommunications operators from the value chain.

INC has the potential to improve the overall system performance in Next Generation Networks Infrastructures (NGNI) by reducing processing time and increasing bandwidth efficiency. INC is steadily changing ``forward-only" routers into server-like devices capable of storing and/or processing incoming data. In other words, as storage and computing grow more affordable, in-network devices will be able to function as standalone servers more frequently. Hence, as computation and caching become new functionalities for ISPs, the network neutrality regulations will need to be reevaluated.  
Note that the regulations will affect the rules on which computing tasks should be transferred to INC devices and which should be retained. This can be handled by Complex Event Processing (CEP) ~\cite{9293092} by transforming the application-specific function into some simple ``match-action" processes for capturing and analyzing data streams to figure out what went wrong (i.e., complex events). Another example is a system created in \cite{9629226} that pools mid-path storage and connects resources to transport data across the end-to-end path. Along the way from the original server to the client, data can transfer from one hop to the next with this new system. It contains a set of mechanisms that ensures: (i) zero packet loss in intermediate network routers, (ii) network stability, and (iii) higher link utilization.
 
 \subsubsection{Privacy}
In cloud computing, the information from all originating nodes is unnecessarily provided to the final destination, which may also create a privacy concern. In this aspect, INC presents a practical trade-off by achieving a privacy-preserving delivery ratio that is near to the ideal. The permission of distributed learning can be provided by subnetworks. Because there are no protocol boundaries between devices when they are all part of the same broadcast domain, imposing security policies is difficult. By breaking up a single large broadcast domain into multiple smaller broadcast domains, a boundary between devices is created.
 
 \subsubsection{Legal and Ethics}
INC will be essential in the support of immersive experience services. Immersive services require even more personal data such as physical attributes of the person to be shared in order to provide a customized service.  Legal and ethical conundrum exits on how this information will be anonymized but it can still be used for customized services.  Although the technical issue of machines for resolving ethical quandaries in the real world is clarified, a society-wide dispute may be necessary to consider and accept the protocols and rules for such services~\cite{8662743}. 
%
%Efficient training of deep learning models necessitates rich data, which is often collected from many sources. This gives an advantage in INC that rich data can be combined in a centralized data center, but because of serious privacy concerns, transmitting sensitive data directly to a single centralized entity for training is not always possible. Furthermore, the data aggregator must adhere to strict data standards. This can be resolved by training the DL model over centralized and encrypted data. With the aim of creating a design for security and utility of distributed knowledge in machine learning, a new protocol called SEDML is introduced in \cite{gao2021sedml}. SEDML is structured on lightweight cryptography. This method is shown to guarantee strong protection for single label prediction while the data is aggregated securely. Throughout the secure gathering procedure, the cloud servers only learn if there is a consensus among the teacher models for a training example. Figure~\ref{fig:SEDML} shows the system architecture of SEDML, a dispensed knowledge in machine learning which is efficiently and securely harnessed.
%\begin{figure}[b]
%\includegraphics[scale=0.4]{Figures/SEDML.png}
%\caption{SEDML system architecture}
%\label{fig:SEDML}
%\end{figure}
%Some machine learning models may have concerns about social inequities and unfairness in the decision-making process. To address this, the designed model shall allow fairness-aware learning. A method is proposed in \cite{anahideh2021choice} for sampling models with varying fairness metrics that are both efficient and effective. Experiments are carried out utilizing real-world benchmark datasets and a variety of classifiers.
%
There are also detailed questions to be resolved, such as the appropriate legal framework when it may be necessary to reveal some of the data or its analysis. Examples include accident data for cars, medical malpractice, and criminal conspiracy.

\subsubsection{Safety and Trust}
An INC node must ensure that the service requests are generated from genuine end-user devices. At the same time, there must be a mechanism to measure the trust of a computing, caching, or control service as well as what are the primary attributes that define the trust of the service. Mainly, a two-way trust relationship is desirable to develop a trusted interaction between INC nodes and end-user devices. An opinion-based model is helpful to choose a computing, caching, or control service. However, the reliability will become an essential factor to be considered. 
%SLA between a cloud service and end-users is limited if the service is processed in the INC. A professional and licensed third-party should monitor SLA verification for end-users and small organizations who lack in technical capability. Although a service provider offers attributes to measure the trust of the service, at the same time, the verification and monitoring of these attributes are not yet studied in detail.


The integration of blockchain with the INC has the potential to enable end-to-end service delivery across the whole ecosystem. Without relying on an intermediary blockchain provides a distributed, unchangeable, single source of truth that everyone agrees with. When INC meets blockchain, two challenges of INC evolve with the advancement of NGNI because of geographically distributed edge nodes and those having limited capabilities. These two challenges that need to be handled are: (i) the assurance of multi-domain resource integration's trustworthiness, and (ii) the overall schedule of heterogeneous and geographically distributed edge and INC resources. For the first challenge, to assure reliability and traceability, blockchain has to be integrated with edge computing and INC. 
%However, most of the work for this focuses solely on the reliability of information, ignoring the trust difficulties that arise throughout the resource allocation process. For the second challenge, some research on the design of a blockchain-based resource management framework is still ongoing. These works, on the other hand, do not address the issue of trust. As a result, the deep aggregation of network resources may be realized compared with challenges. A modular and configurable framework for trusted data management is proposed in \cite{8789542}. The edge device layer, blockchain network layer, and edge nodes layer are all part of this architecture. The mutual authentication protocol, security-enhanced consensus, and smart contracts, as well as block and transaction data management, are all investigated. Blockchain can be adopted by INC to guarantee the information reliability as well as traceability  of transactions, and multidomain resource management is supported by virtual technology, which is widely referred to as network function virtualization. An architecture that addresses heterogeneous resource trust management can be the first one under the background of blockchain meeting INC.


%The degree to which a system is used by different levels of the community is characterized as accessibility. Accuracy, completeness at the point of creation, consistency, and objectivity are all characteristics of trust. Durability is a system attribute that allows software to be available for an extended period~\cite{8768490}. 
The use of INC and blockchain technology can effectively remove the requirement for trust in regulatory compliance. Removing the requirement for trust in regulatory compliance has a challenging technical-legal problem on top of a strong reliance on trust. It can be done by providing access to immutable data to both quality control authorities and enterprises. This will allow control authorities and enterprises to participate more fully in the process. 


\subsubsection{Commercial}\label{INC_business}
INC is an inherently heterogeneous and distributed system and it is possible that different components are governed by independent and competitive autonomous entities.  When in-network computing is performed the cost/benefit should be shared by the related parties.  Although incentive designs and cooperative games are used extensively in the literature for efficient distributed resource allocation in the networks \cite{zhan2020incentive, tang2020communication}, INC introduces additional challenges to be resolved.  These challenges mainly arise due to the scale of operations in INC and it includes efficient and scalable accounting, authentication of operations to be completed, sharing of the incentives (which can be non-monetary).  

Table~\ref{table:Challenges_RSE}, classifies the above discussed papers according to the keywords which they are all mentioned directly or indirectly in papers. Finally, Table~\ref{tab:Acronyms_RSE} gives the acronyms used this section.

%\subsection{NGNI Beyond Shannon Communications }
%\noindent In their seminal work, Shannon and Weaver~\cite{shannon_weaver_1949} categorized communication into three levels based on the purpose of communication; \textit{Level A: Technical}, \textit{Level B: Semantic}, and \textit{Level C: Effectiveness}. At the time, Shannon focused on the technical problem of communicating symbols accurately, and so did the researchers for the following seven decades. Recently, with the increasing differentiation of applications envisioned for 6G, and the soaring need for high bandwidth, there is an emerging interest in the other two types of communications. Semantic communications focus on transferring only the bits that are significant to convey the meaning. With effective communication, the focus is on delivering only the bits that are significant to ensure the receiver takes the action intended by the sender. 
%With both approaches, the core concern is context-specific rather than the error-free delivery of all information symbols, and it is possible to reduce the number of bits transferred by eliminating the bits that are redundant for the application.

%The INC paradigm establishes an opportunity to investigate the problem of semantic and goal-oriented communication in the NGNI. Eliminating the redundancy at the sender may be performed via {\em semantic encoding} at the sender, i.e., determining the next symbol based on the freshness, precision, timeliness and completeness attributes of the information \cite{9475174, uysal2021semantic}. With this approach, communication aims to ensure the sender and receiver are in the same state. 
%Another approach is to determine the next symbol for the sender, based on an estimate of the receiver's understanding of the message. This would be possible via constructing a knowledge base~\cite{CALVANESESTRINATI2021107930} or a knowledge graph~\cite{chein:lirmm-00355336} that is shared between the communicating entities. 
%Such a system typically consists of a computational ontology (providing symbolic representations), facts, rules, and constraints~\cite{chein:lirmm-00355336}, as well as a reasoning engine built on the rules and constraints associated with the given application domain~\cite{CALVANESESTRINATI2021107930}. %The goal of the reasoning engine is to answer questions posed within the application domain.

%The knowledge, which is available at the receiver to interpret the received symbols, is a dynamic notion. In \cite{9530497}, an AI model is used to represent this relationship, and it is trained via coordinated collaboration among edge servers that perform encoding and decoding based on the commonly shared knowledge base. In such architecture, different edge servers can establish and maintain shared AI models without exposing any of their local data uploaded by the users. 

%The cognition of the amount and type of knowledge available to the intended recipient, i.e., the interlocutor, is a determining factor in the message symbols that will be transmitted. In \cite{seo2021semanticsnative}, contextual reasoning is infused into semantics-native communication, such that each speaker agent runs internal simulations by locally and iteratively reasoning about the communication context of the target receiver. Measuring the communication reliability by the receiver's success of correctly recognizing and interpreting the intended message, the expected semantic representation (SR) bit length is derived, which quantifies the extracted effective semantics. Contextual reasoning, i.e., the collection, modeling, reasoning, and distribution of context in relation to sensor data, has also been shown to play a critical role for the Internet of Things (especially for machine-to-machine communications)~\cite{6512846}. In this study, it is argued that the functionalities need to be divided into layers and components in a meaningful manner, such that each component performs a limited subset of the task, and almost independently from the rest.

%Post-Shannon communications are one driving factor towards bringing machine learning together with semantics in network architecture design. Novel deep learning algorithms for knowledge representation in different fields, e.g., speech~\cite{ZeroShotLearn_speech}, image~\cite{CompositionalObverter}, etc., may need to be implemented in the core to reduce end-to-end latencies in communication. In return, the developments in deep learning are the key factor behind the success of post-Shannon communications as such algorithms enable identifying the relevant information at the sender or reducing ambiguity at the receiver, thus improving the goal effectiveness of the communications. Split learning techniques~\cite{gupta2018distributed} may be implemented for speeding up model convergence and improving communication success while preserving communications' confidentiality.


%\subsection{Computation-Caching oriented context-aware Communications } 
 
%\noindent Current and future applications such as federated learning and extended reality have unique requirements that contribute in shifting the focus of network infrastructure researchers from communication-only features to multiple services and functions. Authors of \cite{8869705} advocate that, starting from 6G, network infrastructures must deliver multiple services (i.e., communication, computing, control, and others). That means there must be a tight integration and management of these multiple services while reaching the target performance of each one of them (e.g., computing latency,  stability, etc.). 
%This shift from communication-focused networking has also been supported by the authors of \cite{8808168}, where they proposed a Computation Oriented Communication (COC) service type. This proposed service is supposed to provide an acceptable rate-latency-reliability balance on computation tasks to achieve a certain computational accuracy. The same authors also proposed a Contextually Agile eMBB (enhanced mobile broadband) Communication (CAeC) service type, which is supposed to adapt the provision of eMBB services based on the network context (i.e., link congestion, network topology, or even surrounding physical location and mobility).

%That said, we believe the requirements of NGNI will be even more stringent. By activating INC and the tight integration of 3C/4C, it would be possible for NGNI to offer 3C/4C services throughout the whole Cloud-Edge-Mist Continuum. The provision of these services must be managed according to the availability of 3C resources, but also according to other aspects related to the network and physical context (i.e., link congestion, network topology, mobility, etc.). Given that NGNI will be composed of many distributed and heterogeneous devices belonging to different stakeholders, these latter would also need to cooperate with each other to realize an optimal context-aware 4C service provision. Although this cooperation could be achieved with a compensation or reward-driven approach after solving the convention pricing system challenge discussed in Subsection~\ref{INC_business}, it still adds to the complexity of the problem in hand. That said, realizing a computation-caching oriented context-aware communication that offers 4C services throughout the whole continuum is still an open challenge that needs to be adequately tackled. 
 
%\subsection{Autonomous Networking}
%\noindent Autonomous network management is the holy grail for telecommunication operators. 
%Network autonomy (or automation) could help operators improve a network’s cost-efficiency, %(for reducing maintenance costs), as well as bring flexibility, resilience, ability to bring innovation to market faster, scalability (for different deployments and services), and enhanced security~\cite{NA:whitepaper}. In-network computing allows implementing network functions inside the network. This facilitates in-network control, where the control can be implemented directly inside the network. 
%This idea was proposed in \cite{10.11452740070.2626316}, where it has been argued that datacenter fabric load balancing is best done in the network instead of the transport layer. They have shown that the multipath transport protocol, MPTCP~\cite{10.11452043164.2018467}, is effective for load balancing, but it cannot be implemented in the data center as some applications (e.g., high-performance storage systems) bypass the kernel. In \cite{10.11452740070.2626316}, the authors then proposed a network-based distributed congestion-aware load balancing mechanism for data centers with a global scheme for handling asymmetry and demonstrated that it outperforms MPTCP on a data center testbed. 
%In \cite{10.55553154630.3154637}, the authors performed network resource allocation in hardware (referred to as ``{\em FlexSwitches}''). In \cite{10.11453185467.3185476}, a distributed heavy-hitter detection mechanism is proposed, providing 70\% savings in communication overhead compared to an existing scheme. In \cite{9387694}, the authors proposed an architecture for performing network control functions such as load balancing, congestion control, denial of service attack detection using in-network functions. % MORE DETAILS NEED TO BE ADDED HERE

%To serve traffic workloads efficiently, both service providers and researchers seek ways to enable flexible and demand-aware networking that can exploit the specific spatio-temporal structure of the demand. 
%Demand-aware transportation system has been studied in \cite{9537675}. In a setting with an evolving set of requests for transportation from an origin to a destination before a deadline, the authors study the spatial-temporal demand forecasting and competitive supply (SOUP) problem  and propose a solution that predicts future requests and assigns routes that take into account both the available spatial-temporal request information and the supply-demand state. 
%With the increasing ISP traffic being dominated by a small number of large CDNs connecting at multiple locations, a demand-aware CDN-ISP infrastructure has been proposed in \cite{9566292}. The study was carried out on a large European ISP data, and it revealed that the reconfigurable infrastructure has the potential to reduce backbone capacity by 15\% while reducing path lengths by 30\%, on average and during the critical peak hour. 
%As traffic in data centers grows significantly due to the extensive usage of cloud technologies, the data center network becomes a critical infrastructure for Internet traffic.
%For increased flexibility in the traffic pattern and load that can be serviced by the data center,  free-space optical communications~\cite{10.1145/2619239.2626328} and more recently, optical circuit switches~\cite{10.1145/3098822.3098838} have been utilized, and scalable performance has been demonstrated on proof-of-concept deployments. In \cite{10.1145/3310165.3310170}, the theoretical bounds of demand-aware, {\em self-adjusting} networks have been analyzed.
%The emerging paradigm of utilizing programmable switches in data centers to dynamically adjust their topology based on dynamic traffic demands is investigated in \cite{10.1145/3447868}. 




%\begin{figure}[tb]
%\includegraphics[width=\linewidth]{Figures/ZSM_reference.pdf}
%\caption{The reference architecture for the ZSM framework}
%\label{fig:ZSM_reference}
%\end{figure}

%Recently, due to its importance for %the forthcoming post-5G networks, this topic gained attention from both the research community and international standardization %and industry research organizations. TM Forum’s Zero-touch Orchestration, Operations, and Management (ZOOM)~\cite{TM}, ETSI ZSM (Zero-touch network and Service Management)~\cite{ZSM:intent}, ETSI ENI  ISG (Experiential Network Intelligence Industry Specification Group)~\cite{ETSI}, Open Network Automation Platform (ONAP)~\cite{ONAP}, ITU Focus Group on Autonomous Networks (FG-AN)~\cite{FGAN} bring together different market players to outline the architectures and mechanisms that can achieve the goal of autonomous networks. 

%The aim of network automation is to provide zero-touch network management that requires no human involvement. Artificial intelligence is a key enabler to facilitate self-management. As an example, at the heart of the ZSM framework reference architecture (Figure~\ref{fig:ZSM_reference}) lie intelligent and cognitive {\em closed-loops} (CLs) capable of learning the optimal behavior through interaction with the network~\cite{ZSM:intent}. 
%Machine learning methods allow these CLs to adapt to the changing conditions dynamically and thus help to maintain a robust and flexible network. Another pillar of autonomous networking via the ZSM architecture is modularity (comprising self-contained, loosely coupled services) and the use of {\em intent}-based interfaces. Intents are declarative policies that allow network operators to provide requirements at a high level to simplify and improve the agility of the operations. The intents comprise logical functions that implement data collection, processing, and analysis; these functions are connected to create a machine learning pipeline to provide policy-based network/service automation, thus constituting the Intent-Based Networking (IBN) and closed-loop automation solutions~\cite{9627829}. 


==> Content/driving_use_cases.tex <==
\section{Driving Use Cases for Next-Generation Networking Infrastructure} \label{sec:UseCases}
% \section{Driving Use Cases for NGN}

\noindent In-Network Computing has the potential to shape the Next-Generation Networking Infrastructure (NGNI) into an integrated computation and communication infrastructure that is  needed  to fulfill the stringent requirements of emerging applications. The enhancement of 3C integration throughout Cloud-Edge-Mist Continuum provides even further advantages to achieve this goal. Thus, to highlight the necessity of enabling INC with 3C integration, we present in this section some of the key use cases which prove the limits of current network infrastructure. We also emphasize, for each use case, the features that INC and 3C should provide to fulfill their requirements.

% Next-Generation Networking Infrastructure (NGNI) will explore new and innovative application use cases based on the convergence of different technologies (edge-cloud computing and in-network computing) and the integration of communication, computation, and caching functionalities. Some potential use cases for NGNI are multisensory extended reality (XR) applications, holographic and haptic applications, connected robots and autonomous systems, entertainment, and e-health. Although these cases have been proposed to be enabled by the current network (e.g., 4G/5G), the diversity and stringent requirements of those applications cannot yet be fully met. These high demands impose a reshaping of current network infrastructure towards an NGNI acting as a truly distributed, collaborative, and pervasive system that enables the execution of application-specific tasks and storage of data contents in the Cloud-Edge-Mist continuum with high QoS/QoE guarantees. In the remaining of this section, we present some driving use cases for NGNI and highlight their system requirements.

% \textcolor{blue} {Next-Generation Networking (NGN) will explore new and innovative application use cases based on the convergence of different technologies (edge-fog-cloud computing and in-network computing and caching) and the integration of communication, computation, and caching functionalities. Potential driven cases for NGN are multisensory extended reality (XR) applications, connected robots and autonomous systems, wireless brain-computer interfaces, holographic and haptic applications, entertainment, and e-health. In this section, some of these use cases are discussed.}

 \subsection{Multisensory Extended Reality (XR) Applications}
 
\noindent We are witnessing the evolution of AR/VR applications into a full immersive eXtended Reality (XR) experience that captures multi-modal human sensory information, including sight, hearing, touch, smell, taste, and even emotion~\cite{8869705,9369324}. The applications of XR include remote surgery, immersive education, and gaming.
%In this context, multi-modal human sensory information  should be exchanged between remote receivers in order to support real-time interactions between users in a combined real and virtual application environment (e.g., remote surgery, immersive gaming).

Multisensory XR applications require not only engineering (i.e., communication, computing, caching) requirements but also perceptual requirements (e.g., human senses, cognition, and physiology)~\cite{8869705,9369324}. In the engineering context, these applications require high data rates (1 -- 1000 Gbps), ultra-low latency (0.1 -- 1 ms), and high reliability (99.999 -- 99.99999 \%) due to the vast amount of data generated and human sensitivity~\cite{8329628,9369324}. However,  4G and 5G networks cannot support these applications because they do not incorporate the joint management of 3C functionality. 
Hence, NGNI has the potential to fulfill this void. Consequently, INC allows a certain extent of data analysis such as aggregation, de-duplication, filtering, and preprocessing to be performed \textit{inside} the network as the data traverses the network core. Performing these operations on-the-fly will help reduce the latency and decrease network load. Edge computing may complement INC to deliver content and offload computation-intensive tasks such as AR/VR video coding and decoding and content rendering, further improving the latency and throughput. Finally, collaboration among network nodes allows data content and computation tasks to be replicated and distributed within the network, increasing end-to-end reliability.

Enabling multisensory XR applications introduces several challenges to be overcome.  From a technical perspective,  cross-layer architectures and resource management schemes that seamlessly and efficiently integrate 3C functionality in the NGNI should be designed.  Accordingly, new data compression schemes, data streaming management, and synchronization are required and need further investigation.  Note that considering multisensory communications brings forth the question of how best to relay the meaning of the content rather than how to deliver symbols accurately, i.e., a subject currently investigated in the literature as \textit{Post-Shannon communications}~\cite{CALVANESESTRINATI2021107930}.

Furthermore, multisensory XR inherently involves strictly personal information and processing it inside the network requires further attention to privacy and legal aspects.  Additionally, differentiating the incoming traffic by processing them inside the network requires a revisit to open internet regulations. In particular, Internet Service Providers (ISPs) should have the necessary economic incentives to replace routers with INC devices.

%  \subsection{Wireless Brain-Computer Interfaces}
 
% Brain-Computer Interface (BCI) provides a new form of communication for humans by using their thoughts to interact and control external devices and the environment (e.g., turn on a light, control prosthetic limbs). BCI usually involves electrode sensors to record neuronal activity, communication technologies to transmit the signals, and algorithms to translate those signals into commands relayed to external devices that perform the desired actions. However, traditional BCI systems with wire connections to transmit the monitored brain’s signals are bulky and not user-friendly, thus restricting their use in experimental laboratories. Therefore, removing wire connections with wireless technologies enhances portability and wearability, enabling new and innovative applications (e.g., brain-controlled movies, fully-fledged multibrain-controlled cinemas~\cite{zioga2018enheduanna}). Like XR, wireless BCU requires high data rates, ultra-low latency, high reliability, as well as powerful computation capability~\cite{8869705,9369324}.

 \subsection{Holographic and Haptic Applications}
 
 \noindent Holographic and haptic communications are new forms of interactions expected in the future. Holographic communication consists of capturing, in real-time, information (e.g., images and sounds) of people and objects and sending them to remote locations where they will be projected on the real world using 3D holographic displays. Moreover, to fully realize an immersive experience, haptic feedback can be integrated into holographic applications. In a haptic interaction, haptic devices (e.g., sensors and actuators) capable of sensing and delivering cutaneous, haptic, and kinesthetic feedback enable users to feel, touch and manipulate virtual and remote objects. For instance, remote repair applications can allow technicians to interact with holographic images of real objects located in remote and inaccessible places~\cite{9078581}. As the amount of data necessary to stream the holographic media is significant, holographic and haptic communications require high throughput in the range of hundreds of gigabits per second or even terabits per second. Besides, these communications require ultra-low latency and high reliability because a jitter of more than microseconds immediately degrades holographic and haptic interactions~\cite{9078581,9178307}.
 
As described in XR application case, NGNI is a promising way to meet the strict requirements of holographic and haptic interactions by integrating communication, computation, and caching within the network. Therefore, in-network computing and caching enable holographic and haptic-related computation tasks (e.g., big data analysis, 3D video rendering) and contents (e.g., holographic video) to be placed close to their users to reduce latencies and increase data rates.

Effectively transmitting and processing multimodal data streams, such as audio, holographic, and haptic, is a challenging task that requires 3C integration due to the high demand of these different modalities in terms of transmission delay, jitter, rate, and reliability. This challenge is further aggravated when the users (e.g., surrounding location and current viewpoint) and network contexts (e.g., network congestion and topology) can change over time. Moreover, similar to XR, in-network computing of private personal information requires research into privacy and legal issues.  Furthermore, as haptic communication may be used for applications such as remote surgery, the safety of end-users becomes an important aspect for this type of communication.  Finally, haptic communications will enable remote control of physical systems, and as such, an integrated design of end-system control policies jointly with 3C protocols will be needed.
 
 \subsection{Distributed Machine Learning Applications}
 
 \noindent AI/ML enabling intelligent systems has emerged as a key technology benefiting many aspects of our daily life. Currently, most data-driven systems collect data from local devices and then train the data at centralized cloud data centers. However, user privacy, application latency, and network congestion are major concerns of these centralized intelligent systems. To address these issues, distributed and collaborative learning schemes with the most famous one being federated learning, have received considerable attention. In most of these schemes, local workers only share their built machine learning models instead of sending their raw data to a centralized server. Consequently, these distributed schemes have many benefits in terms of data storage, data acquisition, and privacy presentation by not exchanging raw data. 

Although communication overhead is mitigated in distributed learning schemes, the network is still a major performance bottleneck, especially for large-scale systems, due to two main reasons~\cite{sapio2020scaling,dinh2021innetwork}. First, local workers produce intense bursts of traffic to communicate their model updates as the size of these exchanged models can be very large from hundreds of megabytes to a few gigabytes~\cite{dinh2021innetwork}.  Second, as the centralized server needs to wait to receive the local models from all workers, straggling workers have high latency or slow local training can dramatically stagnate the whole training process. Therefore, large-scale distributed learning requires low latency and high data rates.

By integrating 3C functionality in the whole Cloud-Edge-Mist Continuum, NGNI can be a promising solution to support the two phases of large-scale distributed learning. In essence, distributed learning alternates compute-intensive local training phases with communication-intensive model update synchronization. In the first phase, local training can be performed in edge nodes close to the data sources, as shown in Figure~\ref{fig:FL_with_INC}. Then, in the synchronization phase, intermediate network nodes can execute aggregation operations over models with multiple local workers as these models flow towards the centralized server. In addition, in-network caching can quickly deliver the updated global model to local workers. As a result, in-network computing and caching increase throughput, diminish latency, and speed up training time~\cite{sapio2020scaling,dinh2021innetwork}. 

 \begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{Figures/FL_with_INC.pdf}
    \caption{Distributed Machine Learning with INC.}
    \label{fig:FL_with_INC}
\end{figure}

Security and privacy are major problems of implementing distributed learning in the NGNI. As network nodes can belong to different entities, not all of them are trusted, and even some nodes may be malicious and attack the training process. Regarding privacy issues, computation, offloading and data processing at network nodes may still involve the transmission of potentially sensitive personal data, discouraging privacy-sensitive applications from taking part in model training in the NGNI. A privacy breach can still be incurred when raw data is not exchanged between local workers because private information can be extracted from the shared trained models and parameters. Hence, it is critical to develop 3C solutions in the NGNI that preserve privacy and security while maintaining efficiency. Another challenge facing the practical implementation of distributed learning is that local workers may be reluctant to participate in the learning process without receiving some incentive as the training model is a resource-consuming task.
	
 
 \subsection{Connected Robots and Autonomous Systems}
 
 \noindent Automation, robotics, and autonomous systems (e.g., drones, autonomous cars, robots) are being used to facilitate a variety of vertical domains (e.g., agriculture, automotive, smart factories, and smart cities) and transform our daily life. Leveraging the full potential of such systems introduces many challenges that today’s networks cannot fulfill. Hereafter, we discuss two domains enabled by such systems and driving the development of NGNI.
 
 \subsubsection{Automotive/Vehicular} 
 
\noindent With the rapid growth of urbanization and industrialization, Intelligent Transportation System (ITS) has received increasing interest from industry and academia. ITS plays a crucial key role in providing innovative services to assist traffic authorities efficiently managing traffic flow, making the roads safer, less congested, and reducing emissions. Connected and Autonomous Vehicles (CAVs) are expected to be one of the main building blocks of future smart cities. Indeed, CAVs are equipped with various sensors (e.g., cameras, LiDar, radar, and GPS), communication modules, and on-board units with computing and storage capabilities that enable a wide range of applications. Accordingly, ITS system is a highly dynamic and data-intensive system with stringent delay and reliability requirements. NGNI has the potential to provide high reliability (\textgreater 99.999 \%) and ultra low latency (\textless 1 ms) with high throughput (\textgreater 100 Gbps) necessary for safe functioning of ITS systems~\cite{8869705,9369324}.

With the integration of CAVs resources with those of the NGNI by using Vehicle-to-Vehicle (V2V) and Vehicle-to-Infrastructure (V2I) collaboration, NGNI should be able to provide high reliability in addition to low latency and high throughput for different ITS services. For instance, comprehensive information from the vehicle’s on-board sensor and from the infrastructure (e.g., traffic lights, cameras) can be collected and processed by networked devices such as  road-side units or mobile base stations  to quickly issue warning signals to vehicles with potential safety hazards and assist vehicle safety drive. In-vehicular infotainment (e.g., traffic and weather reports, high-definition maps, and entertainment videos) is another ITS service that can be improved by caching content and offloading related processing tasks (e.g., video transcoding) within the network~\cite{DZIYAUDDIN2021108228}.

The highly dynamic nature of ITS together with the reliability of communications affecting the safety of humans appear as the main challenges.  INC can provide significant flexibility and efficiency of ITS operations by processing vast data as it traverses the network.  However, as the data processed reflects upon the traffic safety, regulations should be put in place to allow all parties involved in ITS to take responsibility for their actions.  Furthermore, the processing of data may also open up new ethical challenges that need to be resolved.  For example, a quick hazard response may save lives but causes financial burden by delaying the traffic in certain areas.  Therefore, 3C resource management techniques to support high-speed vehicles and massive connectivity in ITS systems need further investigation. 
 
 \subsubsection{Industry 4.0} 
 
\noindent The ongoing digital transformation of manufacturing and supply chains that is characterized by a high level of automation and industrial integration through information and communication technologies (e.g., IoT, cyber-physical systems, mobile networks, and cloud computing) is aptly termed as Industry 4.0. Industry automation realizes the control of processes, devices, and systems through a network of sensors and actuators to improve productivity, flexibility, and efficiency in a cost-effective way. This automation comes with rigorous requirements across the rate-reliability-latency spectrum, a balance that is not yet available in today’s networks but which should be in NGNI~\cite{8869705,9178307}. 

NGNI has the potential to enable reliable and real-time control applications (e.g., robotic motion control~\cite{9293092}, industrial assembly~\cite{9468247}) for Industry 4.0 with the help of INC. Data-related operations can be conducted as the measured data flows over the network towards the control decision process, thereby reducing network traffic and increasing throughput.  Control decisions can be performed in network nodes closer to the factory equipment to reduce data path length and processing latencies. Moreover, by supporting collaboration among network nodes, distributed control techniques can be used to improve reliability and latency.  To support a high level of automation for industrial applications or other autonomous systems with stringent requirements, autonomous network management that exploits the interdependence between computing, caching, communication, and control is crucial and quite challenging. Furthermore, distributed control techniques and intelligent decision-making methods require more research investigations to enable full autonomous factories.
 
 \subsection{Entertainment}
 
\noindent The continued growth of video streaming and the widespread use of ultra-high-definition devices  will lead to an unprecedented traffic demand for ultra- and high-quality videos~\cite{rufino20216g}. In particular, 8K video streaming requires four times the bitrate of the 4K video format, which already requires at least the double bitrate of current HD videos, which may have video bitrates up to 15 Mbps. Moreover, the bitrate for streaming non-2D video formats (e.g., $360^\circ$ VR video) can be even higher. However, this high video traffic demand may cause heavy congestion in the current network. Note that video streaming has several important differences compared to the XR and holographic communications discussed earlier.  In video streaming, the data transmitted is not generated in real time and the initial delay is usually not that important, which allows the use of caches in the network for data delivery.  In-network caching can alleviate this traffic burden on the network core by delivering video content within a few hops to the users. Furthermore, on-demand video transcoding within the network allows a fast adaptation to the current user's network conditions, thus improving the user's QoE. Therefore, in-network caching and computing are promising features of NGNI to support the evolution of video streaming.
 
 Another entertainment application that will benefit from NGNI is cloud gaming, a type of online gaming that runs a game on a remote location (e.g., a cloud datacenter) and streams it as a video to end-user devices. Cloud gaming is a computation-intensive application that requires reliable (99.99 \%), high bandwidth (15 -- 500 Mbps), and low latency (\textless  100 ms) communication for an immersive experience~\cite{9464920}. By offloading the rendering and other tasks (e.g., game logic) to distributed computation nodes within the network, cloud gaming may leverage 3C resources to guarantee users’ QoE~\cite{8685768}. For online multi-player games, these nodes should also be able to synchronize the shared game logic.
 
 As entertainment applications are expected to generate massive data traffic in the NGNI, advanced techniques to offload such large data traffic are required. Designing these techniques can be quite challenging due to the heterogeneity and dynamicity of the  3C resources available in the Cloud-Edge-Mist continuum.  The dynamicity of user demands also necessitates these 3C resources to be rented on demand as the need arises, requiring further research into network-wide pricing policies.  The pricing policies should be designed to be both efficient and incentive-compatible.
 
 \subsection{E-Health}
 
\noindent NGNI can help expand the healthcare sector, eliminating time and physical location barriers through diverse remote healthcare services, such as remote monitoring, diagnosis, prevention, treatment, and even remote surgery. For example, doctors can diagnose patients remotely by controlling robots while receiving haptic, audio, and holographic feedback. However, healthcare applications are generally time-sensitive (sub-millisecond latency) and require high-reliable (up to 99.99999 \%) communications~\cite{9040264}. 
With the convergence and collaboration between technologies such as wireless body area networks, edge-cloud computing, and in-network computing technologies, NGNI will enable quick and reliable transportation and processing of large volume of medical data from sensor devices placed closed to, attached on, or implanted inside the human body. 
%Then, real-time health information can be provided from these collected data with the help of AI, in-network computing, and caching. 

Similar to distributed learning applications, security and privacy are major challenges for the e-Health case. As the patient’s health information should be carefully stored and considered sensitive, reliable and secure computing, caching, and communication services are essential. Besides, trust and security mechanisms are required to guarantee that the collected health information from patients is genuine and  malicious attacks on this information are prevented.
 
%  \subsection{Discussion}

% Although the aforementioned or similar application use cases have been proposed to be enabled by the current network (e.g., 4G/5G), the diversity and stringent requirements of those applications cannot be fully met in the current network. These high demands impose a reshaping of current network infrastructure towards an NGN with seamless end-to-end integration of communication, computation, and caching functionalities since individual functionalities affect each other as well as the final outcome in terms of system performance. In this regard, edge-fog-cloud computing and in-network computing are promising concepts to offer communication, caching, and computing functionalities at different parts of the NGN infrastructure. Therefore, NGN can be seen as a truly distributed, cooperative, and pervasive system that enables the execution of application-specific tasks and storage of data contents within the network with high QoS/QoE guarantees.
 

 


==> Content/old_table_INC_def.tex <==
\begin{table*}[t]
\centering
\begin{adjustbox}{width=\textwidth,center=\textwidth}
\resizebox{0.5\textwidth}{!}{\begin{tabular}{c ccc cccc cccc} 

   \toprule 
\multirow{3}{*}{\textbf{Research}}  
       & \multicolumn{3}{c}{\textbf{Definition of INC}} & \multicolumn{4}{c}{\textbf{In Switch $X$}}& \multicolumn{4}{c}{\textbf{Where to Process/Compute}}   \\ 
   \cmidrule(lr){2-4} \cmidrule(lr){5-8} \cmidrule(lr){9-12} 
       & In Network   & In Network   &    In Switch X    & Aggregation  & Caching  & Traffic  & Other  & Conventional   & Programmable & Virtual/Physical  & Delegated/Offloaded    \\ 
       
        &  Processing & Computing  &        &   &   & Processing & operations & devices  & devices&  middelboxes & to devices   \\ 
        
   \midrule 
\multirow{1}{*}{\cite{ports2019should}}   
 
       &      & \checkmark     &    &      &      &    &      &      & \checkmark     & \checkmark     &    \\ 
        %\addlinespace 
        \hline
       \multirow{1}{*}{\cite{blocher2021holistic}}  
      
       &      & \checkmark    &      &      &      &    &      &      &   \checkmark     &      &            \\ 
        %\addlinespace 
        \hline
        \multirow{1}{*}{\cite{mustard2019jumpgate}}  
      
       & \checkmark    &      &      &      &      &    &    &      &  \checkmark     &      &             \\ 
        %\addlinespace   
        \hline
          \multirow{1}{*}{\cite{mai2014netagg}}  
      
       & \checkmark    &     &      & \checkmark     &        &  &        &        &      & \checkmark     &             \\ 
        %\addlinespace 
        \hline
          \multirow{1}{*}{\cite{anwer2015programming}}  
      
       & \checkmark  &     &    &      &      &\checkmark     &      &      &     &    \checkmark   &             \\ 
        %\addlinespace 
        \hline
          \multirow{1}{*}{\cite{sapio2017network}}  
      
       &      & \checkmark      &     &      &      &   &      &  \checkmark    &     &     &          \checkmark   \\ 
        %\addlinespace 
        \hline
          \multirow{1}{*}{\cite{tokusashi2018lake}}  
      
       &      & \checkmark    &      &      &      &  &       &    & \checkmark     &    &  \\ 
              %\addlinespace 
                \hline
         \multirow{1}{*}{\cite{Zilberman}}  

       &      & \checkmark    &      &      &      &    &      &  \checkmark    &     & \checkmark    &             \\ 
        %\addlinespace 
        \hline
          \multirow{1}{*}{\cite{INC6G}}  
      
       &    &     \checkmark   &      &  \checkmark    &  \checkmark    &   \checkmark  &     &      &      & \checkmark    &             \\ 
        %\addlinespace 
        \hline
          \multirow{1}{*}{\cite{alim2016flick} }  
      
       & \checkmark     &      &      &      &      &   &   \checkmark    &      &    \checkmark   &      &             \\ 
       %\addlinespace 
       \hline
          \multirow{1}{*}{\cite{zhang2014smartswitch}}  
      
       & \checkmark     &      &      &  \checkmark    &    &    &  \checkmark   &  \checkmark    &    \checkmark    &     &             \\ 
     
        
   \bottomrule 
\end{tabular}} 
 \end{adjustbox}
 
 \caption{INC Definition Classification}
\label{table:1}
\end{table*}

